How Do Java Developers Reuse StackOverflow Answers in Their GitHub Projects?

StackOverflow (SO) is a widely used question-and-answer (Q\&A) website for software developers and computer scientists. GitHub is an online development platform used for storing, tracking, and collaborating on software projects. Prior work relates the information mined from both platforms to link user accounts or compare developers' activities across platforms. However, not much work is done to characterize the SO answers reused by GitHub projects. For this paper, we did an empirical study by mining the SO answers reused by Java projects available on GitHub. We created a hybrid approach of clone detection, keyword-based search, and manual inspection, to identify the answer(s) actually leveraged by developers. Based on the identified answers, we further studied topics of the discussion threads, answer characteristics (e.g., scores, ages, code lengths, and text lengths), and developers' reuse practices. We observed that most reused answers offer programs to implement specific coding tasks. Among all analyzed SO discussion threads, the reused answers often have relatively higher scores, older ages, longer code, and longer text than unused answers. In only 9% of scenarios (40/430), developers fully copied answer code for reuse. In the remaining scenarios, they reused partial code or created brand new code from scratch. Our study characterized 130 SO discussion threads referred to by Java developers in 357 GitHub projects. Our empirical findings can guide SO answerers to provide better answers, and shed lights on future research related to SO and GitHub.

==> discussion.tex <==
\section{Our Recommendations}

%Our work reveals the SO answer code reused by developers. It classifies the answer code based on topics of discussion threads, and shows that the majority of discussion threads are about coding tasks or optimizations
%Our work reveals the SO answers reused by developers. It classifies the answers based on topics of discussion threads, and shows that the majority of those threads are about coding tasks or optimizations. It also classifies SO answers based on developers' reuse practices, showing that 
Our work reveals the SO answers reused by developers, and characterized those answers from different aspects. 
%It characterizes the question style and technical content for any discussion threads holding those answers (see Findings 1 \& 2). It contrasts the reused as well as unused answers from the same discussion threads in terms of score, age, code length, and text length (see Finding 3). It also classifies developers' reuse practices for those answers (see Finding 4). 
Based on this study, we provide the following recommendations: 
%Our empirical findings led to the following recommendations.

\textbf{For people wanting to quickly earn points by answering questions: } Answerers should provide complete and/or optimized solutions to questions (see Finding 1).  They should prioritize questions on data processing, feature implementation in a certain context, inspection/manipulation of program execution at runtime, or file processing, because many questions/threads on these topics were reused (see Finding 2).

\textbf{For people searching SO for technical solutions: }If it is hard to choose the best answer among alternatives, people can focus more on the answers with higher scores, longer code, and/or longer answers, because such answers are more likely to be better and get reused by other people (see Finding 3).  

\textbf{For tool developers: }According to Finding 4, future tools can relate SO answers with the GitHub code reusing them. For instance, when people view an SO answer, their browsers will also present GitHub code reusing that answer to demonstrate the answer usage and customization. Additionally, future tools can customize developer-selected SO answers for specific program contexts. With Finding 2, we recommend future tools to generate programs from the natural-language descriptions of popular and/or error-prone tasks. Tool builders can even compare the effectiveness between such tools and existing tools (e.g.,  ChatGPT~\cite{chatgpt} and GitHub Copilot~\cite{copilot}).

\textbf{For researchers looking for reused answers: }With Finding 4, we recommend researchers not to solely rely on clone detection tools to restore the connections between SO answers and GitHub codebases. Because developers often do not cite the SO answers they reuse (Section~\ref{sec:reuse}), researchers should not solely search for code citing answer IDs either. 

\textbf{For programmers who reused SO answers: }Properly cite answer IDs to give credits to answerers, improve program comprehension, and facilitate data analytics by researchers.
%data analytics by researchers.
